GFM-RAG: Graph Foundation Model for Retrieval Augmented Generation

Retrieval-augmented generation (RAG) has proven effective in integrating knowledge into large language models (LLMs). However, conventional RAGs struggle to capture complex relationships between pieces of knowledge, limiting their performance in intricate reasoning that requires integrating knowledge from multiple sources. Recently, graph-enhanced retrieval augmented generation (GraphRAG) builds graph structure to explicitly model these relationships, enabling more effective and efficient retrievers. Nevertheless, its performance is still hindered by the noise and incompleteness within the graph structure. To address this, we introduce GFM-RAG, a novel graph foundation model (GFM) for retrieval augmented generation. GFM-RAG is powered by an innovative graph neural network that reasons over graph structure to capture complex query-knowledge relationships. The GFM with 8M parameters undergoes a two-stage training process on large-scale datasets, comprising 60 knowledge graphs with over 14M triples and 700k documents. This results in impressive performance and generalizability for GFM-RAG, making it the first graph foundation model applicable to unseen datasets for retrieval without any fine-tuning required. Extensive experiments on three multi-hop QA datasets and seven domain-specific RAG datasets demonstrate that GFM-RAG achieves state-of-the-art performance while maintaining efficiency and alignment with neural scaling laws, highlighting its potential for further improvement.

==> figures/radar.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=2.5in]{images/radar.pdf}
    \vspace{-.4cm}
    \caption{Model performance and generalizability comparison.}
    \label{fig:radar}
    \vspace{-0.7cm}
\end{figure}

==> figures/scaling.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=2.3in]{images/scaling_law.pdf}
    \vspace{-.3cm}
    \caption{Neural scaling law of \ourmethod.}
    \label{fig:scaling}
    \vspace{-.6cm}
\end{figure}

==> sections/4_preliminary.tex <==
\section{Preliminary}\label{sec:preliminary}
Given a set of documents $\gD=\{D_1,D_2,\ldots,D_{|\gD|}\}$, we can construct a knowledge graph $\gG=\{(e,r,e')\in \gE\times\gR\times\gE\}$, where $e\in\gE$ and $r\in\gR$ denote the set of entities and relations extracted from $\gD$, respectively. 

\noindent\textbf{GraphRAG Framework.} 
Given a user query $q$, we aim to design a graph-enhanced retriever to obtain relevant documents from $\gD$ by leveraging the knowledge graph $\gG$. The whole GraphRAG process  can be formulated as:
\begin{gather}
    \gG = \text{Construct}(\gD), \\ \gD^K = \text{Graph-retriever}(q,\gD,\gG),\\
    a = \text{LLM}(q,\gD^K),
\end{gather}
where $\gD^K$ denotes the top-$K$ retrieved documents and $a$ denotes the final answer generated by large language models (LLMs). In this paper, we design a novel graph retriever, a GFM retriever, which will be described in detail next.
